Efficient Image Restoration via Latent Consistency Flow Matching

Recent advances in generative image restoration (IR) have demonstrated impressive results. However, these methods are hindered by their substantial size and computational demands, rendering them unsuitable for deployment on edge devices. This work introduces ELIR, an Efficient Latent Image Restoration method. ELIR addresses the distortion-perception trade-off within the latent space and produces high-quality images using a latent consistency flow-based model. In addition, ELIR introduces an efficient and lightweight architecture. Consequently, ELIR is 4$\times$ smaller and faster than state-of-the-art diffusion and flow-based approaches for blind face restoration, enabling a deployment on resource-constrained devices. Comprehensive evaluations of various image restoration tasks and datasets show that ELIR achieves competitive performance compared to state-of-the-art methods, effectively balancing distortion and perceptual quality metrics while significantly reducing model size and computational cost. The code is available at: https://github.com/eladc-git/ELIR

==> files/theory.tex <==
\newcommand{\aset}[1]{\left\{#1\right\}}
\newcommand{\xhat}{\widehat{X}}
\newcommand{\xstar}{X^*}
\newcommand{\zhat}{\widehat{Z}}
\newcommand{\ztilde}{\widetilde{Z}}
\newcommand{\zstar}{Z^*}
\newcommand{\xtilde}{\widetilde{X}}
\section{Theoretical Results}


\begin{equation}
    D\brackets{P}=\min\limits_{p_{\xhat|Y}}\aset{\expectation{\norm{X-\xhat}^2}{}: W_2\brackets{p_{X},p_{\xhat}}\leq P},
\end{equation}
where 


In this work we assume a given decoder that $\xhat=\mathcal{D}_{\Theta}\brackets{\zhat}$ is are result of a latent representation $\zhat$ and re-frame the problem as follows:
\begin{align}\label{eq:problem_latent}
    D_{L}\brackets{P}&=\min\limits_{\substack{p_{\zhat|Y}}}\aset{\expectation{\norm{X-\mathcal{D}_{\Theta}\brackets{\zhat}}_2}{}: W_2\brackets{X,\xhat}\leq P, \xhat=\mathcal{D}_{\Theta}\brackets{\zhat}}.
        % &=\min\limits_{p_{\zhat|Y}}\aset{\expectation{\norm{X-\mathcal{D}\brackets{\zhat}}^2}{}: W_2\brackets{X,\xhat}^2\leq P^2, \xhat=\mathcal{D}\brackets{\zhat}}
\end{align}

Next, we would like to find $\Theta$ and $p_{Z_1|Y}$  which address problem \eqref{eq:problem_latent}. 


\subsection{Bound}
Let $\zstar=g_{\Omega}\brackets{Y}$ be the latent minimal mean square error estimator (MMSE), meaning:
\begin{align}
    \zstar\brackets{Y}=\arg\min\limits_{g}\expectation{\norm{X-\mathcal{D}\brackets{g\brackets{Y}}}^2}{X,Y}
\end{align}
\begin{align}\label{eq:error_decompostion_latent}
    \expectation{\norm{X-\mathcal{D}\brackets{\zhat}}^2}{}&=\expectation{\norm{\mathcal{D}\brackets{\zstar}-\mathcal{D}\brackets{\zhat}}^2}{X,Y}+\expectation{\norm{X-\mathcal{D}\brackets{\zstar}}^2}{X,Y}\\
    &-2\expectation{\brackets{X-\mathcal{D}\brackets{\zstar}}^T\brackets{\mathcal{D}\brackets{\zstar}-\mathcal{D}\brackets{\zhat}}}{X,Y}\nonumber
    % &\leq \expectation{\norm{\mathcal{D}\brackets{\zstar}-\mathcal{D}\brackets{\zhat}}^2}{}+\expectation{\norm{X-\mathcal{D}\brackets{\zstar}}^2}{}\\
    % &+2\expectation{\norm{X-\mathcal{D}\brackets{\zstar}}\norm{\mathcal{D}\brackets{\zstar}-\mathcal{D}\brackets{\zhat}}}{X,Y}\\
    % &\leq \expectation{\norm{\mathcal{D}\brackets{\zstar}-\mathcal{D}\brackets{\zhat}}^2}{}+\expectation{\norm{X-\mathcal{D}\brackets{\zstar}}^2}{}\\
    % &+2\sqrt{\expectation{\norm{X-\mathcal{D}\brackets{\zstar}}^2}{} \expectation{\norm{\mathcal{D}\brackets{\zstar}-\mathcal{D}\brackets{\zhat}}^2}{}}
\end{align}


\begin{align}
    &2\expectation{\brackets{X-\mathcal{D}\brackets{\zstar}}^T\brackets{\mathcal{D}\brackets{\zstar}-\mathcal{D}\brackets{\zhat}}}{X,Y}=\\
    &2\expectation{\brackets{X-\mathcal{D}\brackets{\tilde{Z}}}^T\brackets{\mathcal{D}\brackets{\zstar}-\mathcal{D}\brackets{\zhat}}}{X,Y}\\
    &+2\expectation{\brackets{\mathcal{D}\brackets{\tilde{Z}}-\mathcal{D}\brackets{\zstar}}^T\brackets{\mathcal{D}\brackets{\zstar}-\mathcal{D}\brackets{\zhat}}}{X,Y}
\end{align}
where $\tilde{Z}=\mathcal{E}\brackets{X}$


\begin{align}
    D\brackets{P}&\leq D_{LMMSE}+\min\limits_{p_{\zhat|Y}}\aset{\expectation{\norm{\mathcal{D}\brackets{g_{\Omega}\brackets{Y}}-\mathcal{D}\brackets{\zhat}}^2}{\zhat,Y}: W_2\brackets{X,\xhat}\leq P, \xhat=\mathcal{D}\brackets{\zhat}},
        % &\leq \expectation{\norm{X-\mathcal{D}\brackets{g_{\Omega}\brackets{Y}}}^2}{}+\min\limits_{p_{\zhat|Y}}\aset{\expectation{\norm{\mathcal{D}\brackets{g_{\Omega}\brackets{Y}}-\mathcal{D}\brackets{\zhat}}^2}{\zhat,Y}}
    % &= \expectation{\norm{X-\mathcal{D}\brackets{\zstar}}^2}{}+\min\limits_{p_{\zhat|\zstar}}\aset{\expectation{\norm{\mathcal{D}\brackets{\zstar}-\xhat}^2}{}: W_2\brackets{X,\xhat}\leq P, \xhat=\mathcal{D}\brackets{\zhat}}
\end{align}
where $D_{LMMSE}\triangleq\expectation{\norm{X-\mathcal{D}_{0}\brackets{g_{\Omega}\brackets{Y}}}^2}{}$ is the latent  MMSE estimator error. Since $g_{\Omega}$ is a deterministic function of $Y$ we can re frame the problem \eqref{} as follows:
\begin{align}
    D\brackets{P}&\leq D_{LMMSE}+\min\limits_{\substack{p_{\zhat|\ztilde}\\ \Theta}}\aset{\expectation{\norm{\mathcal{D}_0\brackets{\ztilde}-\xhat}^2}{\zhat,\ztilde}: W_2\brackets{X,\xhat}\leq P, \xhat=\mathcal{D}_{\Theta}\brackets{\zhat_1}},
\end{align}



In the next part we wise 

\todo[inline]{Not sure about the next part !!}

Next, we investigate the Wasserstein distance  
\begin{align}
    W_2\brackets{X,\xhat}\leq W_2\brackets{X,\xtilde}+W_2\brackets{\xtilde,\xhat}
\end{align}
where $\xtilde=\mathcal{D}_{0}\brackets{\mathcal{E}_{0}\brackets{X}}$ is the sample $X$ with encoder-decoder error.  Utilizing the Wasserstein distances we have:
\begin{align}
    W_2\brackets{X,\xtilde}&\triangleq \brackets{\inf\limits_{\nu\in\Pi\brackets{X,\xtilde}}\int_{\mathcal{X}\times\mathcal{X}}\norm{x-\tilde{x}}^p d\nu\brackets{x,\tilde{x}}}^{\frac{1}{2}}=\brackets{\inf\limits_{\nu\in\Pi\brackets{X,\xtilde}}\int_{\mathcal{X}\times\mathcal{X}}\norm{\tilde{x}-\tilde{x}+\Delta_{\mathcal{E}\mathcal{D}}\brackets{x}}^p d\nu\brackets{x,\tilde{x}}}^{\frac{1}{2}}\\
    &\leq \sqrt{\expectation{\norm{\Delta_{\mathcal{E}\mathcal{D}}\brackets{x}}^2}{X}}
\end{align}
Plugging \eqref{} and \eqref{} into \eqref{} results in 
\begin{align}
    D\brackets{P}&\leq \expectation{\norm{X-\mathcal{D}\brackets{g_{\Omega}\brackets{Y}}}^2}{}+\min\limits_{p_{\zhat|Y}}\aset{\expectation{\norm{\mathcal{D}\brackets{g_{\Omega}\brackets{Y}}-\mathcal{D}\brackets{\zhat}}^2}{\zhat,Y}: W_2\brackets{\xtilde,\xhat}\leq P_{\mathcal{E}\mathcal{D}}, \xhat=\mathcal{D}\brackets{\zhat}},
        % &\leq \expectation{\norm{X-\mathcal{D}\brackets{g_{\Omega}\brackets{Y}}}^2}{}+\min\limits_{p_{\zhat|Y}}\aset{\expectation{\norm{\mathcal{D}\brackets{g_{\Omega}\brackets{Y}}-\mathcal{D}\brackets{\zhat}}^2}{\zhat,Y}}
    % &= \expectation{\norm{X-\mathcal{D}\brackets{\zstar}}^2}{}+\min\limits_{p_{\zhat|\zstar}}\aset{\expectation{\norm{\mathcal{D}\brackets{\zstar}-\xhat}^2}{}: W_2\brackets{X,\xhat}\leq P, \xhat=\mathcal{D}\brackets{\zhat}}
\end{align}
where $P_{\mathcal{E}\mathcal{D}}=P-\sqrt{\expectation{\norm{\Delta_{\mathcal{E}\mathcal{D}}\brackets{x}}^2}{X}}$

\todo[inline]{
\begin{align}
    W_p\brackets{X,Y}\triangleq \brackets{\inf\limits_{\nu\in\Pi\brackets{X,Y}}\int_{\mathcal{X}\times\mathcal{X}}\norm{x-y}^p d\nu\brackets{x,y}}^{\frac{1}{p}}
\end{align}}

\begin{align}
    D\brackets{P}&\leq \expectation{\norm{X-\mathcal{D}\brackets{g_{\Omega}\brackets{Y}}}^2}{}+\min\limits_{p_{\zhat|\zstar}}\aset{\expectation{\norm{\mathcal{D}\brackets{\zstar}-\mathcal{D}\brackets{\zhat}}^2}{\zhat,\zstar}: W_2\brackets{\ztilde,\zhat}\leq \frac{P_{\mathcal{E}\mathcal{D}}}{L_{\mathcal{D}}}},
        % &\leq \expectation{\norm{X-\mathcal{D}\brackets{g_{\Omega}\brackets{Y}}}^2}{}+\min\limits_{p_{\zhat|Y}}\aset{\expectation{\norm{\mathcal{D}\brackets{g_{\Omega}\brackets{Y}}-\mathcal{D}\brackets{\zhat}}^2}{\zhat,Y}}
    % &= \expectation{\norm{X-\mathcal{D}\brackets{\zstar}}^2}{}+\min\limits_{p_{\zhat|\zstar}}\aset{\expectation{\norm{\mathcal{D}\brackets{\zstar}-\xhat}^2}{}: W_2\brackets{X,\xhat}\leq P, \xhat=\mathcal{D}\brackets{\zhat}}
\end{align}
% For $P=0$ we have:
% \begin{align}
%     D\brackets{P}&\leq \expectation{\norm{X-\mathcal{D}\brackets{g_{\Omega}\brackets{Y}}}^2}{}+\min\limits_{p_{\zhat|Y}}\aset{\expectation{\norm{\mathcal{D}\brackets{g_{\Omega}\brackets{Y}}-\mathcal{D}\brackets{\zhat}}^2}{\zhat,Y}: W_2\brackets{X,\mathcal{D}\brackets{\zhat}}=0}
% \end{align}
\subsection{Optimalitiy codontion}
\begin{align}\label{eq:error_decompostion}
    \expectation{\norm{X-\mathcal{D}\brackets{\zhat}}^2}{}=\expectation{\norm{\xstar-\mathcal{D}\brackets{\zhat}}^2}{}+\expectation{\norm{X-\xstar}^2}{}-2\expectation{\brackets{X-\xstar}^T\brackets{\xstar-\mathcal{D}\brackets{\zhat}}}{}.
\end{align}
where $\xstar=\expectation{X|Y}{}$ is the minimal mean square error estimator (MMSE). 
\begin{align}\label{eq:croos_zero}
    \expectation{\brackets{X-\xstar}^T\brackets{\xstar-\mathcal{D}\brackets{\zhat}}}{}&=\expectation{\expectation{\brackets{X-\xstar}^T\brackets{\xstar-\mathcal{D}\brackets{\zhat}}|Y}{}}{}\\
    &=\expectation{\expectation{\brackets{X-\xstar}^T|Y}{}\expectation{\brackets{\xstar-\mathcal{D}\brackets{\zhat}}|Y}{}}{}=0.
\end{align}
In the first step, we utilized the law of total expectation and in the second step we use the fact that $\xstar$ is a deterministic function $Y$ and $\xhat$ is independent of $X$ given $Y$.
Combining \eqref{eq:croos_zero}, \eqref{eq:error_decompostion} and plunging into \eqref{eq:problem_latent} results in:
\begin{equation}
    D\brackets{P}=D^*+\min\limits_{p_{\zhat|Y}}\aset{\expectation{\norm{\xstar-\mathcal{D}\brackets{\zhat}}^2}{}: W_2\brackets{p_{X},p_{\mathcal{D}\brackets{\zhat}}}\leq P},
\end{equation}
where $D^*\triangleq\expectation{\norm{X-\xstar}^2}{}$ is the MMSE estimator error.  




\section{Theoretical Results V2}


Starting from the optimal 2-stage solution:
\begin{equation}\label{eq:problem_latent2}
    D\brackets{P}=D^* + \min\limits_{p_{\xhat}}\aset{W_2^2\brackets{p_{\xhat},p_{\xstar}}: W_2\brackets{p_{\xhat},p_{X}}\leq P},
\end{equation}
where $D^*\triangleq\expectation{\norm{X-\xstar}^2}{}$ is the MMSE estimator.  


Let's define sub optimal estimator $\bar{X}=\mathcal{D}(g(\mathcal{E}(Y)))=\mathcal{D}(Z^*)$:
\begin{align}\label{eq:inq_mmse}
  D^*=\expectation{\norm{X-\xstar}^2}{} \leq \expectation{\norm{X-\bar{X}}^2}{} = \expectation{\norm{X-\mathcal{D}(g(\mathcal{E}(Y)))}^2}{}
\end{align}

Inequality 20 from \cite{dao2023flow}
\begin{align}\label{eq:inq_w2}
    W_2^2\brackets{p_{\xhat},p_{\xstar}} \leq \norm{\Delta_{\mathcal{E},\mathcal{D}}}^2 + \Delta_{\zstar \rightarrow \zhat}
\end{align}

\begin{align}\label{eq:inq_w2_2}
    W_2^2\brackets{p_{\xhat},p_{X}} \leq \norm{\Delta_{\mathcal{E},\mathcal{D}}}^2 + \Delta_{\zhat \rightarrow Z} \triangleq P^2
\end{align}

Putting \eqref{eq:inq_mmse}, \eqref{eq:inq_w2} and \eqref{eq:inq_w2_2} in \eqref{eq:problem_latent2}, we can express $D\brackets{P}$ for $\norm{\Delta_{\mathcal{E},\mathcal{D}}}^2 + \Delta_{\zhat \rightarrow Z} \leq P$:
\begin{align}\label{eq:inq}
    D\brackets{P} &\leq \expectation{\norm{X-\mathcal{D}(g(\mathcal{E}(Y)))}^2}{} +  \min\limits_{p_{\xhat}}\aset{\norm{\Delta_{\mathcal{E},\mathcal{D}}}^2 + \Delta_{\zstar \rightarrow \zhat}: W_2\brackets{p_{\xhat},p_{X}}\leq P}\\
    &\leq \expectation{\norm{X-\mathcal{D}(g(\mathcal{E}(Y)))}^2}{} +  \min\limits_{p_{\mathcal{D}(\zhat)}}\aset{\Delta_{\zstar \rightarrow \zhat}} + \norm{\Delta_{\mathcal{E},\mathcal{D}}}^2
\end{align}


